Capturing and Animation of Body and Clothing from Monocular Video

While recent work has shown progress on extracting clothed 3D human avatars from a single image, video, or a set of 3D scans, several limitations remain. Most methods use a holistic representation to jointly model the body and clothing, which means that the clothing and body cannot be separated for applications like virtual try-on. Other methods separately model the body and clothing, but they require training from a large set of 3D clothed human meshes obtained from 3D/4D scanners or physics simulations. Our insight is that the body and clothing have different modeling requirements. While the body is well represented by a mesh-based parametric 3D model, implicit representations and neural radiance fields are better suited to capturing the large variety in shape and appearance present in clothing. Building on this insight, we propose SCARF (Segmented Clothed Avatar Radiance Field), a hybrid model combining a mesh-based body with a neural radiance field. Integrating the mesh into the volumetric rendering in combination with a differentiable rasterizer enables us to optimize SCARF directly from monocular videos, without any 3D supervision. The hybrid modeling enables SCARF to (i) animate the clothed body avatar by changing body poses (including hand articulation and facial expressions), (ii) synthesize novel views of the avatar, and (iii) transfer clothing between avatars in virtual try-on applications. We demonstrate that SCARF reconstructs clothing with higher visual quality than existing methods, that the clothing deforms with changing body pose and body shape, and that clothing can be successfully transferred between avatars of different subjects. The code and models are available at https://github.com/YadiraF/SCARF.

==> preliminaries.tex <==
\section{Preliminaries}
\label{FLAMEDECODER}

\qheading{Geometry prior:}
FLAME~\cite{FLAME2017} is a statistical 3D head model that combines separate linear identity shape and expression spaces with \ac{LBS} and pose-dependent corrective blendshapes to articulate the neck, jaw, and eyeballs.
Given parameters of facial identity $\shapecoeff \in \mathbb{R}^\shapedim$, pose $\posecoeff \in \mathbb{R}^{3\numjoints+3}$ (with $\numjoints=4$ joints for neck, jaw, and eyeballs), and expression $\expcoeff \in \mathbb{R}^\expdim$, FLAME outputs a mesh with $\numverts=5023$ vertices. 
The model is defined as
\begin{equation}
\flamev(\shapecoeff, \posecoeff, \expcoeff) = W(T_P(\shapecoeff, \posecoeff, \expcoeff),  \joints(\shapecoeff), \posecoeff, \blendweights),
\end{equation}
with the blend skinning function $W(\template, \joints, \posecoeff, \blendweights)$ that rotates the vertices in $\template \in \mathbb{R}^{3\numverts}$ around joints $\joints \in \mathbb{R}^{3\numjoints}$, linearly smoothed by blendweights $\blendweights \in \mathbb{R}^{\numjoints \times \numverts}$. The joint locations $\joints$ are defined as a function of the identity $\shapecoeff$. Further,
\begin{equation}
T_P(\shapecoeff, \posecoeff, \expcoeff) = \template + B_S(\shapecoeff; \shapespace) + B_P(\posecoeff; \posespace) + B_E(\expcoeff; \expspace)
\end{equation}
denotes the mean template $\template$ in ``zero pose'' with added shape blendshapes $B_S(\shapecoeff; \shapespace): \mathbb{R}^{\shapedim} \rightarrow \mathbb{R}^{3\numverts}$, pose correctives $B_P(\posecoeff; \posespace): \mathbb{R}^{3\numjoints+3} \rightarrow \mathbb{R}^{3\numverts}$, and expression blendshapes $B_E(\expcoeff; \expspace): \mathbb{R}^{\expdim} \rightarrow \mathbb{R}^{3\numverts}$, with the learned identity, pose, and expression bases (i.e.~linear subspaces) $\shapespace, \posespace$ and $\expspace$. See~\cite{FLAME2017} for details.

\qheading{Appearance model:}
FLAME does not have an appearance model, hence we convert the Basel Face Model's linear albedo subspace \cite{Paysan2009} into the FLAME UV layout to make it compatible with FLAME.
The appearance model outputs a UV albedo map $\albedo(\albedocoeffs) \in \mathbb{R}^{\uvsize \times \uvsize \times 3}$ for albedo parameters $\albedocoeffs \in \mathbb{R}^{\albedodim}$.

\qheading{Camera model:}
Photographs in existing in-the-wild face datasets are often taken from a distance.
We, therefore, use an orthographic camera model $\cam$ to project the 3D mesh into image space. 
Face vertices are projected into the image as $\vect{v} = s\Pi(\flamev_i)+\vect{t}$, where $\flamev_i \in \mathbb{R}^3$ is a vertex in $\flamev$, $\Pi \in \mathbb{R}^{2 \times 3}$ is the orthographic 3D-2D projection matrix, and $s \in \mathbb{R}$ and $\vect{t} \in \mathbb{R}^2$ denote isotropic scale and 2D translation, respectively.
The parameters $s$, and $\vect{t}$ are summarized as $\boldsymbol{c}$.

\qheading{Illumination model:}
For face reconstruction, the most frequently-employed illumination model %
is based on Spherical Harmonics (SH)~\cite{Ramamoorthi2001AnER}. 
By assuming that the light source is distant and the face's surface reflectance is Lambertian, the shaded face image is computed as:
\begin{equation}
    B(\albedocoeffs, \lighting, \normals_{uv})_{i,j} = \albedo(\albedocoeffs)_{i,j} \odot \sum_{k = 1}^{9}{\lighting_{k} H_{k}(\normals_{i,j})},
\end{equation}
where the albedo, $\albedo$, surface normals, $\normals$, and shaded texture, $B$, are represented in UV coordinates %
and where $B_{i,j} \in \mathbb{R}^3$, $\albedo_{i,j} \in \mathbb{R}^3$, and $\normals_{i,j} \in \mathbb{R}^3$ denote pixel $(i,j)$ in the UV coordinate system. %
The SH basis and coefficients are defined as $H_k: \mathbb{R}^3 \rightarrow \mathbb{R}$ and $\lighting = [\lighting_{1}^T, \cdots, \lighting_{9}^T]^T$, with $\lighting_{k} \in \mathbb{R}^3$, and $\odot$ denotes the Hadamard product. 

\qheading{Texture rendering:}
Given the geometry parameters ($\shapecoeff, \posecoeff, \expcoeff$), albedo ($\albedocoeffs$), lighting ($\lighting$) and camera information $\boldsymbol{c}$, we can generate the 2D image $\image_r$ by rendering as $\image_r = \mathcal{R}(\flamev, B, \cam)$, where $\mathcal{R}$ denotes the rendering function.
 
FLAME is able to generate the face geometry with various poses, shapes and expressions from a low-dimensional latent space. 
However, the representational power of the model is limited by the low mesh resolution and therefore mid-frequency details are mostly missing from FLAME's surface.
The next section introduces our expres\-sion-dependent displacement model that augments FLAME with mid-frequency details, and it demonstrates how to reconstruct this geometry from a single image and animate it.


